Analog Codes on Graphs

We consider the problem of transmission of a sequence of real data produced by a Nyquist sampled band-limited analog source over a band-limited analog channel, which introduces an additive white Gaussian noise. An analog coding scheme is described, which can achieve a mean-squared error distortion proportional to $(1+SNR)^{-B}$ for a bandwidth expansion factor of $B/R$, where $0 < R < 1$ is the rate of individual component binary codes used in the construction and $B \geq 1$ is an integer. Thus, over a wide range of SNR values, the proposed code performs much better than any single previously known analog coding system.

==> Makefile <==
#################################################################################
#################################################################################
##
## Author: Nandakishore Santhi (nsanthi@ucsd.edu)
##
## This Makefile is meant for use with the following LaTeX(2e) systems:
## (1) Linux + GNU make + (pdf)LaTeX
## (2) Windows + GNU make + MiKTeX
## (3) Windows + cygwin + GNU make + (pdf)LaTeX
##
#################################################################################
#################################################################################
FILE=analogcodes
#Use for Windows + MiKTeX
#TEXOPTIONS=-include-directory=. -include-directory=Styles -include-directory=Sections
#Use for Linux/Unix
TEXOPTIONS=
LATEX=TEXINPUTS=.//:./Styles//:./Sections//:./Support: latex ${TEXOPTIONS}
PDFLATEX=TEXINPUTS=.//:./Styles//:./Sections//:./Support: pdflatex ${TEXOPTIONS}
BIBTEX=bibtex
SOURCES=analogcodes.tex \
		MyMacros.tex \
		MyBiblio.bib

all: ${SOURCES} Makefile
	@make -s pdf ps
	@echo "___________________________________________________________"
	@echo "Check for errors in out_bib.log out_ps.log and out_pdf.log!"
	@echo "___________________________________________________________"

dvi: ${FILE}.dvi
${FILE}.dvi: ${SOURCES}
	${LATEX} ${FILE}.tex
	${BIBTEX} ${FILE} > out_bib.log
	${LATEX} ${FILE}.tex
	${LATEX} ${FILE}.tex > out_ps.log

pdf: ${FILE}.pdf
${FILE}.pdf: ${SOURCES}
	@echo "Patience Pays!"
	${PDFLATEX} ${FILE}.tex
	${BIBTEX} ${FILE} > out_bib.log
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex
	${PDFLATEX} ${FILE}.tex > out_pdf.log
	@echo "___________________________________________________________"

ps: ${FILE}.ps
${FILE}.ps: ${SOURCES}
	@echo "Patience Pays Again!"
	@make dvi
	dvips -Z -V -t letter ${FILE}.dvi -o ${FILE}.ps
	#pdf2ps -dSubsetFonts=true -dPDFSETTINGS=/printer -dEmbedAllFonts=true -dOptimize=true -dEmbedAll=true ${FILE}.pdf
	#acroread -toPostScript -size letter -scale 100 -level3 ${FILE}.pdf
	gzip ${FILE}.ps
	@echo "___________________________________________________________"

close:
	@pdfclose --file ${FILE}.pdf

open:
	@pdfopen --file ${FILE}.pdf

neat:
	@rm -f *.bak *.dvi *.log *.out *.aux *.idx *.lof *.lot *.toc *.blg ./Figs/*.fig.bak

prepare:
	@make neat
	@rm -f *.ps *.ps.gz *.pdf

clean:
	@make neat
	@rm -f *.bbl *.ps *.ps.gz *.pdf

